General Agentic Memory Via Deep Research

Memory is critical for AI agents, yet the widely-adopted static memory, aiming to create readily available memory in advance, is inevitably subject to severe information loss. To address this limitation, we propose a novel framework called \textbf{general agentic memory (GAM)}. GAM follows the principle of "\textbf{just-in time (JIT) compilation}" where it focuses on creating optimized contexts for its client at runtime while keeping only simple but useful memory during the offline stage. To this end, GAM employs a duo-design with the following components. 1) \textbf{Memorizer}, which highlights key historical information using a lightweight memory, while maintaining complete historical information within a universal page-store. 2) \textbf{Researcher}, which retrieves and integrates useful information from the page-store for its online request guided by the pre-constructed memory. This design allows GAM to effectively leverage the agentic capabilities and test-time scalability of frontier large language models (LLMs), while also facilitating end-to-end performance optimization through reinforcement learning. In our experimental study, we demonstrate that GAM achieves substantial improvement on various memory-grounded task completion scenarios against existing memory systems.

==> fromat.tex <==
\section{Submission of papers to NeurIPS 2025}


Please read the instructions below carefully and follow them faithfully.


\subsection{Style}


Papers to be submitted to NeurIPS 2025 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures.
% Additional pages \emph{containing only acknowledgments and references} are allowed.
Additional pages \emph{containing references, checklist, and the optional technical appendices} do not count as content pages.
Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2025 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the website at
\begin{center}
  \url{https://neurips.cc}
\end{center}
The file \verb+neurips_2025.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2025 is \verb+neurips_2025.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2025.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2025+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2025}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2025/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}

\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix

\section{Technical Appendices and Supplementary Material}
Technical appendices with additional results, figures, graphs and proofs may be submitted with the paper submission before the full submission deadline (see above), or as a separate PDF in the ZIP file below before the supplementary material deadline. There is no page limit for the technical appendices.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}


\end{enumerate}

==> src/conclusion.tex <==
\section{Conclusion}

==> src/experiment.tex <==
\section{Experiments}

\subsection{Experimental Setup}
\paragraph{Datasets.} 
We evaluate GAM and all baselines on four benchmarks that collectively capture the essential challenges of long-term agent memory. Specifically, we adopt textbf{LoCoMo}~\cite{locomo}, a conversational memory benchmark that requires the agent to maintain and retrieve information across extended multi-turn interactions; \textbf{HotpotQA}~\cite{hotpotqa}, a widely used multi-hop question answering dataset that tests the integration of evidence from multiple passages; \textbf{LongBench v2}~\cite{longbenchv2}, a suite of long-context tasks spanning diverse domains and designed to probe robustness under extremely long inputs rigorously; \textbf{LongCodeBench}~\cite{longcodebench}, a large-scale benchmark for code understanding in long-context settings, where we restrict our evaluation to the question-answering (QA) subset to focus on memory-intensive reasoning tasks. For LongBench v2 and LongCodeBench, when the input sequence exceeds the maximum context window supported by the underlying backbone models, we follow the official LongBench v2 truncation principle: retaining the first half and the last half of the sequence while discarding the middle portion.



\paragraph{Evaluation Metrics.} Evaluation protocols are aligned with standard practice for each dataset. On LoCoMo, we report both F1 and BLEU-1, which jointly measure factual recall and lexical fidelity across conversational turns. On HotpotQA, we follow the official setup and report F1 as the sole metric for multi-hop QA. For LongBench v2 and LongCodeBench, we adopt accuracy as the unified evaluation criterion.


\paragraph{Baselines.} We compare GAM with the following representative baselines: \textbf{RAG}~\cite{rag}: the standard Retrieval-Augmented Generation paradigm, which retrieves relevant passages from an external corpus and augments the input context. \textbf{MemoryBank}~\cite{memorybank}: a long-term memory mechanism with a dense-retrieval store for dialogue turns/events and an Ebbinghaus-inspired updating/forgetting policy. \textbf{A-Mem}~\cite{amem}: an agentic memory that creates structured notes and dynamic links among previous memories. \textbf{Mem0}~\cite{mem0}: a system that extracts, consolidates, and retrieves salient conversational memories. \textbf{MemoryOS}~\cite{memoryos}: an OS-style hierarchical memory integrating storage, updating, retrieval, and generation modules.


% \paragraph{Implementation Details.}

\subsection{Main Results}
\input{table/main_results}

% \subsection{Ablation Study}


\subsection{Scaling Analysis}

\input{table/scaling_test}



\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figure/scaling_fig.pdf} % 图片文件名和路径
    \caption{Scaling results.} % 图片标题
    \label{fig:method} % 可用于引用的标签
\end{figure}







==> src/introduction.tex <==
\section{Introduction}


Large Language Models (LLMs) have demonstrated remarkable capabilities on various NLP tasks~\cite{}.  A growing research focus is now on building AI agents based on LLMs that perform complex autonomous reasoning and tool use, leading to increasingly longer task sequences and interaction histories~\cite{agent_usage_1,agent_usage_2,agent_usage_3}.
However, their efficacy is constrained by the inherent limitation of fixed-length context windows, which hinders reasoning over long dialogues or documents~\cite{llmcontextwindowlimit}and leads to significant latency and impractical costs~\cite{mem1}. Rather than relying on computationally expensive methods to extend the core context window~\cite{}, recent efforts are increasingly turning to external memory mechanisms to manage long-term context efficiently. 


Recent approaches to memory mechanisms often model memory as an external storage module, employing retrieval methods to query relevant historical contexts. By doing so, they enable the agent to leverage critical information from long-term history without processing it in its entirety, effectively expanding its functional context window~\cite{}. Considerable research has focused on memory storage mechanisms, exploring techniques for efficient context compression~\cite{memgpt,memoryos}, flexible storage updating~\cite{} and organizing history into structured human-defined formats such as knowledge graphs for effective retrieval~\cite{zep,multiplememory}. However, despite these advances in storage, the querying of historical data often remains simplistic, typically relying on single-round search tools like BM25 or embedding-based similarity~\cite{amem,mem0,memoryr1}. Although effective for straightforward scenarios like dialogues, we argue that these methods are inadequate for complex scenarios, such as research assistants, that require multistep reasoning and nuanced synthesis of historical information~\cite{}. Furthermore, while memory compression enhances efficiency, it inevitably incurs information loss, and manually designed storage formats lack the flexibility required for dynamic and complex tasks.

%图上需要注明research agent和memorization agent, session那里没有必要标注split，检索的是最新的几个相关历史event应该体现出来，和历史event的关系也应该符号化



To solve the above problems, we re-examined the design principles of the memory mechanism and proposed an effective automation framework based on it. First, the memory mechanism should include two modules: storage history, including saving history and generating indexes, and utilization history, including in-depth analysis of historical information and integration of answers.

To address these limitations, we introduce an agentic framework for memory management that moves beyond external storage and simple retrieval. We propose Agentic-Mem, which employs a dual-agent architecture (Fig.~\ref{fig:method}) comprising a Memorization Agent and a Research Agent. The Memorization Agent automatically extracts and indexes key events from diverse, complex historical sessions (e.g., conversations, code, web pages), preserving links to the original context to prevent information loss. It also maintains relationships between current and historical events to facilitate causal reasoning between events. For efficiency, it retrieves the most temporally adjacent relevant events, summarizes their relationships, and stores this summary. The Research Agent then handles complex queries through an iterative process of retrieval, reflection, and synthesis. It first analyzes the relationships between retrieved events and historical events to determine if further historical context is needed. It then reflects on whether the gathered information from retrieved events suffices to answer the current query; if not, it generates new search queries and continues a new round of retrieval. This cycle repeats until the query is fully resolved, at which point all information is synthesized into a final response.
This framework enables comprehensive recall of history from extremely long contexts by Research Agent with nearly lossless fidelity by Memorization Agent, effectively simulating the benefit of an infinite context window.
Experimental results on dialogue, question-answering, and code generation datasets show that Agentic-Mem significantly outperforms existing baselines and remains competitive with those granted full context access, validating its effectiveness across diverse scenarios.

Our contributions are summarized as follows:
\begin{itemize}
    \item We propose Agentic-Mem, an agentic framework for memory management that moves beyond external storage and simple retrieval.  It enables comprehensive, nearly lossless utilization of long-term historical context in complex scenarios, effectively simulating an infinite context window.
    \item We introduce a novel Research Agent capable of iterative retrieval, reflection, and synthesis of historical information. Unlike previous static retrieval methods, Research Agent dynamically reasons over multi-step queries, allowing for nuanced comprehension of prolonged interaction histories.
    \item Extensive experiments demonstrate that Agentic-Mem achieves consistently stronger performance than baselines across diverse tasks and remains competitive with those granted full context access.
\end{itemize}

% ################ original text

% Large Language Models (LLMs)-based agents have demonstrated remarkable capabilities of addressing complex and dynamic tasks across diverse domains~\cite{agent_usage_1,agent_usage_2,agent_usage_3}. A key factor underlying this progress is memory: agents must not only recall past interactions, decisions, and environmental signals but also integrate this knowledge into ongoing reasoning and decision-making processes~\cite{memorysurvey}. As use cases grow in scale and complexity, ranging from customer support bo ts to autonomous vehicles and research assistants~\cite{agentdrive,agentdeepresearch}, the demand for reliable and scalable memory has intensified. This need has shifted the memory system from simple storage and recall toward agentic memory—the capacity of an agent to store, recall, and strategically apply relevant information over time.

% Despite its importance, effective memory management in agents presents several challenges. First, the fixed context windows of LLMs limit the agents' ability to directly process or recall all relevant information once these boundaries are exceeded~\cite{llmcontextwindowlimit}. Second, continuously handling vast volumes of context introduces prohibitive computational costs and latency, leading to expensive processing pipelines and undermining system responsiveness~\cite{mem1}. Third, the burden of managing vast amounts of information often falls on a single leading agent, creating bottlenecks and reducing system performance~\cite{metagpt,singleagentmemory}. Addressing these problems requires the development of general agentic memory architectures that are scalable, efficient, and contextually adaptive. Such systems will enable agents to handle complex, long-term interactions without compromising speed, cost, or performance.

% Some recent studies on memory systems for LLM-based agents are largely centered on summarization-based memorization and rule-driven retrieval. Raw contexts are typically compressed into human-defined structures such as notes, knowledge graphs, or structured databases~\cite{memgpt,memoryos,zep,multiplememory}. And retrieval is managed through rule-based pipelines, including methods like BM25 or embedding-based search models, to search for relevant information~\cite{amem,mem0,memoryr1}. While these designs are effective in relatively constrained settings, such as chatbot applications, they face two fundamental limitations for general-purpose agents. First, their reliance on linear summarization and static storage formats makes them suitable only for narrow, relatively predictable conversations, but ill-equipped for dynamic environments requiring multi-step reasoning and long-term context integration. Second, their dependence on handcrafted rules and heavily engineered retrieval pipelines restricts scalability and adaptability, preventing smooth generalization to diverse and evolving use cases.


% To address these limitations, we propose a new paradigm for general agentic memory that emphasizes flexibility, scalability, and minimal manual engineering. At the foundation of our design is a \textit{memorization agent} that processes incoming raw context and compresses it into lightweight, navigable structures, including event-based notes and session summaries, which function as an index over the original information space. These memory representations preserve essential content in a compact form while enabling efficient access. Building on this foundation, a \textit{research agent} serves as the core reasoning engine. Rather than relying on static, rule-based retrieval pipelines, the research agent leverages the indexed memory to actively explore and analyze the raw contextual data as a continuous information space. Equipped with a toolkit of retrieval and reasoning methods such as embeddings, re-ranking, and BM25, it engages in planning, searching, and reflection to dynamically locate, evaluate, and synthesize relevant information. The collaboration between the memorization agent and the research agent thus establishes a clear division of labor: the former maintains organized, navigable memory representations, while the latter performs adaptive investigation and reasoning over both structured memory and raw context, producing coherent and contextually grounded outputs. 


% Through this design, our framework seeks to achieve the central objective of agentic memory: enabling agents to handle long, complex contexts with the same effectiveness as if they had unlimited direct access to their full history, but without incurring prohibitive computational costs or latency. By minimizing handcrafted rules and maximizing adaptability, our approach offers a promising pathway toward scalable memory systems that support robust long-term reasoning in LLM-based agents. 

% \yby{Our contributions are summarized as follows}:
% \begin{itemize}
%     \item We introduce a paradigm for general agentic memory, combining a memorization agent and a research agent to balance efficiency with adaptability.
%     \item We formalize the design principles of agentic memory as moving beyond summarization and retrieval, toward dynamic reasoning over raw and structured contexts.
%     \item Extensive experiments demonstrate that the framework achieves consistently strong performance across diverse tasks and scaling regimes, while retaining the capacity for continual optimization.
% \end{itemize}




==> src/method.tex <==
\section{Method}
%逻辑差不多了，符号体系和语言还需要继续修改


To address the challenges outlined above, we propose an agentic memory framework that builds
on two complementary roles: a Memorization agent that structures and indexes historical context,
and a Research agent that performs deep research on historical context and summarizes the response. Our framework is illustrated in Figure~\ref{fig:method}, and we will describe the details of the framework in this section.

% As illustrated in Figure~\ref{fig:method}, the
% framework enables both persistent organization of memory and iterative, reasoning-driven query
% resolution.

% The memorization agent incrementally transforms raw sessions into structured
% events. Each event is typed and linked to prior events through explicit relations such as temporal
% adjacency or causal connection. This design ensures that memory remains compact, non-redundant,
% and traceable to its source, providing an index for later reasoning and retrieval. The research agent is responsible for adaptive reasoning and retrieval. When a query is issued, it engages in an iterative cycle consisting of (i) Planning, where a retrieval strategy is formulated; (ii) Searching, which collects candidate events from memory using both similarity-based and relation-based exploration; (iii) Reflection, where the sufficiency and coherence of retrieved evidence are evaluated, triggering further rounds if needed; and (iv) Summarizing, which removes redundancy in organized sessions and retains key information.

% This division of labor enables the system to maintain persistent, organized representations of past interactions while supporting flexible, reasoning-driven retrieval. The following sections first define notation and then provide detailed descriptions of each agent.

\subsection{Notation Formulation}
We define the raw content of contextual pages as $\mathcal{R}$, which is a collection of sessions $\mathcal{S}$, where a session is a record of user interactions, including conversations, code snippets, questions and answers, etc. If $M$ conversations occurred historically, then we have:
\begin{equation}
\mathcal{R} = \{S_1, S_2, ..., S_M \}.
\end{equation} 
Note that the sessions here are naturally segmented based on the timing of user interactions. However, for sessions with extremely long text content, we manually segment the sessions into smaller sessions. 
Both Memorization agent and Research agent are LLM-based agents, we denote the prompt-driven LLM function of Memorization agent as $f_{M}(\cdot)$, and the function of Research agent as $f_{R}(\cdot)$. We define the driven prompt format as $\mathcal{P}$, and use subscripts to distinguish different prompts. Memorization Agent maintain a working memory $\mathcal{M}$, which is a collection of events $\mathcal{E}$. A single session may contain multiple events. Assuming that $M$ historical sessions have occurred, containing a total of $N$ events, then we have:
\begin{equation}
\mathcal{M} = \{\mathcal{E}_1, \mathcal{E}_2, ..., \mathcal{E}_N \}.
\end{equation} 
Furthermore, we define the use of tools as a function $\mathcal{T}(\cdot)$. 
Next, starting from the end of the ($M+1$)-th session and the beginning of the ($M+2$)-th session, we will provide a detailed explanation of how our Memorization Agent and Research Agent work.


% \subsection{keep}


% The general process of agentic memory for LLM-based agents can be formalized into two components: memorization and retrieval. At each interaction step $t=1, \cdots, T$, the agent receives a session of context segments $S_t={s_{t,1},s_{t,2},\cdots,s_{t,n}}$, where each segment may denote a user utterance, an environmental observation, or an external knowledge snippet. The accumulated interaction history up to step $t$ is denoted as $S_{1:T}={S_1,S_2,\cdots,S_T}$. 


% Direct reasoning over $S_{1:T}$ is computationally infeasible due to both the quadratic cost of transformer attention and the fixed-length context window of LLMs. To address this, a memory state is defined as $M_t$ that stores structured events distilled from raw sessions. The memory is updated incrementally as $M_t=f(M_{t-1}, S_t)$ where $f$ is an update operator that extracts salient events from the new session and integrates them into the existing memory. Each event is represented as a type unit: $e=(\texttt{id},\texttt{type},\texttt{value})$, where $\texttt{id}$ is the unique identifier, $\texttt{type}$ specifies the semantic category, and $\texttt{value}$ contains the content extracted from $S_t$ and the relationship with other events. Thus, the memory at time $t$ is the set $M_t={e_1,e_2,\cdots,e_m}$. 

% When solving a task, given a query $q$, the system retrieves a set of relevant elements $R_q=g(q,M_t,S_{1:T})$, where $g$ is a retrieval operator that may combine memory $M_t$ with selective exploration of the raw history $S_{1:T}$. Therefore, the final answer can be generated as $A_q=h(R_q)$.

% The design objective of a general agentic memory framework can be formalized along two dimensions: 
% performance equivalence and efficiency.

% \paragraph{Performance Equivalence.} For any query $q$, the memory-augmented answer should 
% be nearly indistinguishable from the result achievable with full access to the 
% uncompressed history $S_{1:T}$. Formally,
% \begin{equation}
% \mathbb{E}_{q \sim \mathcal{Q}} \Big[ \text{score}\big(h(R_q), \, h(q, S_{1:T})\big) \Big] \;\ge\; \delta,
% \end{equation}
% where $\text{score}(\cdot,\cdot)$ denotes a fidelity metric (e.g., accuracy, F1, BLEU), and 
% $\delta \in [0,1]$ is a threshold close to 1. This requirement guarantees that the memory preserves the informational sufficiency of long contexts while avoiding degradation in task performance.

% \paragraph{Efficiency.}
% Let $C(\cdot)$ denote the computational cost of operating on a given input. The system should 
% achieve performance equivalence while satisfying
% \begin{equation}
% C\big(h(R_q)\big) \;\ll\; C\big(h(q, S_{1:T})\big),
% \end{equation}
% ensuring reduced latency, storage overhead, and processing complexity. 

% Together, these two criteria require that agentic memory retain the fidelity of full-context reasoning while providing a scalable and cost-effective alternative to unbounded context processing.


% \subsection{Overview of Agentic Memory}

% To address the challenges outlined above, we propose an agentic memory framework that builds on two complementary roles: a Memorization agent that structures and indexes historical context, and a Research agent that performs adaptive retrieval and reasoning. As illustrated in Figure~\ref{fig:method}, the framework enables both persistent organization of memory and iterative, reasoning-driven query resolution.


% \textbf{Memorization agent.} The memorization agent incrementally transforms raw sessions into structured events. Each event is typed and linked to prior events through explicit relations such as temporal adjacency or causal connection. This design ensures that memory remains compact, non-redundant, and traceable to its source, providing an index for later reasoning and retrieval.


% \textbf{Research agent.} The research agent is responsible for adaptive reasoning and retrieval. When a query is issued, it engages in an iterative cycle consisting of (i) Planning, where a retrieval strategy is formulated; (ii) Searching, which collects candidate events from memory using both similarity-based and relation-based exploration; (iii) Reflection, where the sufficiency and coherence of retrieved evidence are evaluated, triggering further rounds if needed; and (iv) Summarizing, which removes redundancy in organized sessions and retains key information.

% This division of labor enables the system to maintain persistent, organized representations of past interactions while supporting flexible, reasoning-driven retrieval. The following sections provide detailed descriptions of each agent.



% We do not store the raw session data; instead, we extract the data from the session and store it as different events. So as for the storage format of memory, we define it as $\mathcal{M}$, which contains a series of historical events $e$ extracted from historical sessions $\mathcal{S}$:
% \begin{equation}
% \mathcal{M} = \{e_1, e_2, ..., e_N \}.
% \end{equation}


\subsection{Memorization Agent}

The Memorization Agent is responsible for generating and storing an index of historical sessions, facilitating efficient utilization of historical data. Specifically, the complete original session remains in the raw data $\mathcal{R}$, while the Memorization Agent maintains the working memory $\mathcal{M}$. In this working memory, sessions are stored as events. The Memorization Agent generates a short description $t$ for each event and maintains an index $\text{Id}$ of the current session, allowing subsequent retrieval of the original session via the associated event. We use a carefully designed prompt $\mathcal{P}_{\text{event}}$ to drive the Memorization Agent to extract events and automatically generate descriptions. Note that the Memorization Agent uses the current working memory to generate descriptions for events, thus efficiently integrating event information into the continuously evolving memory.
So for the ($M+1$)-th historical session $S_{M+1}$, assuming there are $k$ events, then we have:
\begin{equation}
\begin{aligned}
\mathcal{R} &= \mathcal{R} \cup \{ S_{M+1} \} \\
f_{M}(S_{M+1}, \mathcal{M}, P_{\text{event}}) &= \{ \mathcal{E}_i\}_{i=1}^{i=k}, \quad \text{ where } \mathcal{E}_i = (t_i, \text{Id}=M+1 ) \\
\mathcal{M} &= \mathcal{M} \cup \{ \mathcal{E}_i\}_{i=1}^{i=k}
\end{aligned}
\end{equation}



% The memorization agent is responsible for transforming incoming raw sessions into structured, event-based memory entries. Its operation follows three steps: event extraction, relation construction, and memory update. This pipeline ensures that essential information is retained, explicitly connected to prior knowledge, and efficiently integrated into the evolving memory state.


% Given a new session of context $S_t$, the memorization agent identifies salient information and converts it into a set of events:
% \begin{equation}
% E_t = \phi_{\text{event}}(S_t) = { e_1, e_2, \ldots, e_k }, 
% \end{equation}
% where each event is defined as 
% \begin{equation}
% e = (\texttt{id}, \texttt{type}, \texttt{value}), \quad \texttt{value} = (\texttt{session\_id}, c).
% \end{equation}
% $\texttt{id}$ is a unique identifier, $\texttt{type}$ denotes the semantic category (event, fact, definition, metric, or other), $\texttt{session\_id}$ records the source session, and $c$ denotes the extracted content.

% For each new event $e_j \in E_t$, the agent establishes explicit links with existing events in the memory $M_{t-1}$. These relations are formalized as:
% \begin{equation}
% \mathcal{R}(e_j) = { (e_i, r, e_j) \mid e_i \in M_{t-1}, ; r \in \mathcal{T} },
% \end{equation}
% where $\mathcal{T}$ is the set of relation types, such as temporal adjacency, causal dependency, and semantic association. The content field of each event is then expanded as $\texttt{content} = (c, \mathcal{R}(e_j))$.

% After constructing event-level relations, the new events are integrated into the memory:
% \begin{equation}
% M_t = M_{t-1} \cup E_t.
% \end{equation}
% \yby{Two principles govern the design: (i) \textbf{Relation-awareness}, ensuring that events are explicitly linked to one another through temporal, causal, or semantic relations, rather than stored as isolated entries;
% and (ii) \textbf{Traceability}, ensuring that each memory entry maintains links to its source in $S_{1:t}$ so that the research agent can revisit evidence when necessary.}




\subsection{Research Agent}
% The research agent constitutes the reasoning-centric component of our memory framework. Its primary role is to transform retrieval into a goal-directed investigation rather than a static search, thereby ensuring that evidence selection remains adaptive, relation-aware, and minimally dependent on handcrafted heuristics. The agent operates through an iterative cycle that integrates \textbf{Planning}, \textbf{Search}, \textbf{Reflection}, and \textbf{Summarizing}, as illustrated in Figure~\ref{fig:method}.

The research agent is responsible for retrieving useful historical information by utilizing all available historical data, including working memory $\mathcal{M}$ and the original historical context content $\mathcal{R}$. It accomplishes this by employing a deep-research approach, autonomously \textbf{planning}, \textbf{tools using}, and \textbf{reflection} on the results to find comprehensive relevant historical information. Finally, it conduct \textbf{summarizing} and integrates all the historical information to generate a response.


\paragraph{Planning.} 

For the newly started $(M+2)$-th session, the research agent autonomously plans whether to call a tool or directly conduct summarizing based on the query $\mathcal{Q}$ provided by the working agent maintaining the current session (or context of the current session if no query is provided) and working memory $\mathcal{M}$, using a carefully designed prompt $\mathcal{P}_{\text{plan}}$. If it need more raw contextual information, generate a tool call command $\mathcal{T}$ and parameters $\mathcal{Q}_{\text{tool}}$, otherwise it returns an empty value and conducts summarizing to generate an answer.

% Planning is the stage that converts a user query $q$ into a set of executable search terms, which serve as the starting point for retrieval. Instead of directly applying the query to the memory, the research agent first reformulates it into a structured representation that highlights salient entities, temporal expressions, and relation cues. This step ensures that retrieval is both targeted and sensitive to the event-based structure of memory.

% Formally, given a query $q$, the planning operator generates a search term set , where each $t_i$ is a compact keyword or phrase distilled from $q$. The generation process emphasizes coverage of critical semantic dimensions, such as entities, dates, or relation markers, thereby improving alignment with the stored event representations.

\begin{equation}
\begin{aligned}
    % f_R(\mathcal{Q}, P_{\text{query}}) &= {t_1, t_2, \ldots, t_m} = \{t_{i}\}_{i=1}^{t=m}
    f_R(\mathcal{Q}, \mathcal{M}, \mathcal{P}_{\text{plan}}) = \left\{
    \begin{array}{ll}
        (\mathcal{T}, \mathcal{Q}_{\text{tool}}) & \text{if need more information}  \\
        N/A  & \text{if working memory is enough to answer}
    \end{array}
  \right.
\end{aligned}
\end{equation}


\paragraph{Tool using.} 

% The search stage operationalizes the search terms produced during planning to gather a pool of candidate events from the memory. This process combines direct retrieval with relation-aware expansion to ensure comprehensive coverage of evidence.

% Given the search term set $T(q)$, the research agent first retrieves the Top-k relevant events from the memory $M_t$:
The purpose of tool using is primarily to retrieve relevant information from the raw content of historical session context $\mathcal{R}$ to compensate for any information loss in the working memory $\mathcal{M}$. Here the tool function $\mathcal{T}$ mainly includes two types of tools: one directly retrieves the raw session based on session id, and the other finds relevant sessions based on keywords using bm25. Therefore, the tool call parameters $\mathcal{Q}_{\text{tool}}$ generated during the planning process include both session ID and the keywords to be used for the search.
We will denote the collection of retrieved session documents as $\mathcal{D}$:
\begin{equation}
\begin{aligned}
% R_q^{(0)} = \texttt{Top-}k\big(\texttt{Match}(T(q), M_t)\big),
\mathcal{T}(\mathcal{Q}_{\text{tool}}, \mathcal{R}) &= \mathcal{D},  \mathcal{D} = \{S_1, S_2, ..., S_k \}
\end{aligned}
\end{equation}
% where $\texttt{Match}(\cdot)$ denotes a similarity function between search terms and event content. The set $R_q^{(0)}$ forms the initial evidence pool.


% Through this two-step procedure, the search stage ensures that not only directly matching events but also their relationally connected counterparts are included, thereby uncovering multi-hop evidence chains that are crucial for complex reasoning tasks.

\paragraph{Reflection.}
After obtaining relevant historical sessions through tool calls, the Research Agent uses reflection to determine whether the current information is sufficient to answer the query. If not, it continues to generate tool calling commands and parameters; otherwise, it returns an empty result and proceeds to the next summerizing stage. In this way, the research agent can find the most comprehensive relevant historical information. Therefore, based on the query $\mathcal{Q}$, the current working memory$\mathcal{M}$, and the retrieved session documents $\mathcal{D}$, we have:
% The reflection stage evaluates whether the retrieved evidence pool $R_q$ is sufficient to support answering the query.
% First, the research agent performs a completeness check:
\begin{equation}
\begin{aligned}
% \texttt{if } \neg \texttt{Sufficient}(R_q, q) \quad \Rightarrow \quad T(q) \gets \texttt{Refine}(q, R_q),
f_R(\mathcal{Q}, \mathcal{M}, \mathcal{D}, \mathcal{P}_{\text{reflect}}) = \left\{
    \begin{array}{ll}
        (\mathcal{T}, \mathcal{Q}_{\text{tool}}) & \text{if need more information}  \\
        N/A  & \text{if current searching results is enough to answer}
    \end{array}
  \right.
\end{aligned}
\end{equation}

If the reflection phase generates new tool calling commands and parameters, the tool using process continues, and the newly retrieved session documents are added to the retrieved document collection $\mathcal{D}$:
\begin{equation}
\begin{aligned}
\mathcal{D} = \mathcal{D} \cup \mathcal{T}(\mathcal{Q}_{\text{tool}})
\end{aligned}
\end{equation}
The reflection phase is repeated until the results indicate that the current information is sufficient to answer the question, no new tool calling commands are generated, or the maximum number of reflection iterations is reached.
% where $\texttt{Sufficient}(\cdot)$ measures whether all reasoning hops and critical entities are adequately covered, and $\texttt{Refine}(\cdot)$ produces improved search terms. This mechanism establishes an iterative loop across planning, search, and reflection until adequacy is achieved.

% Once completeness is verified, the reflection stage passes the curated pool forward. In this way, reflection serves as a gatekeeper that ensures only sufficient and coherent evidence is advanced to the summarization phase.


\paragraph{Summarizing.}

% After reflection confirms sufficiency, the summarizing stage condenses the curated evidence into a minimal sufficient set. Its purpose is to eliminate redundancy while retaining all information necessary for downstream reasoning.

% Formally, summarization can be expressed as a compression operator $\sigma(\cdot)$:
Once sufficient relevant historical information has been gathered, the Research Agent summarizes the information generate an answer $\mathcal{A}$ to the current query $\mathcal{Q}$ . As mentioned above, if the working memory $\mathcal{M}$ contains enough information, Research Agent uses this information directly to generate the response; otherwise, it uses the retrieved session documents $\mathcal{D}$ after tool using to summarize and generate the answer.
\begin{equation}
\begin{aligned}
% R_q^{\ast} = \sigma(R_q), \quad R_q^{\ast} \subseteq R_q,
% r = f_R(o, P_{\text{ans}})
% \mathcal{A} = f_R(\mathcal{D}, \mathcal{P}_{\text{summary}})
\mathcal{A} = \left\{
    \begin{array}{ll}
        f_R(\mathcal{D}, \mathcal{Q}, \mathcal{P}_{\text{summary}}) & \text{if } \mathcal{D} \text{ is not N/A}  \\
        f_R(\mathcal{M}, \mathcal{Q}, \mathcal{P}_{\text{summary}})  & \text{if } \mathcal{D} \text{ is N/A}
    \end{array}
  \right.
  \end{aligned}
\end{equation}
% where $R_q^{\ast}$ denotes the minimal subset that preserves informational completeness for answering $q$. The operator $\sigma$ removes duplicated events, merges overlapping content, and prunes irrelevant relations, thereby producing a compact yet sufficient slice of memory.



% \begin{algorithm}[t]

% \caption{Work flow of Research Agent}\label{alg:research_agent}
% \begin{algorithmic}[1]
% \Require{}

% \end{algorithmic}
% \end{algorithm}



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\textwidth]{figure/main_fig.pdf} % 图片文件名和路径
%     \caption{Overview of Agentic Memory.} % 图片标题
%     \label{fig:method} % 可用于引用的标签
% \end{figure}


==> src/related_work.tex <==
\section{Related Work}

%语言还没refine

\paragraph{Memory Augmented LLM Agents}.
Large Language Models (LLMs) have emerged as powerful general-purpose reasoners, capable of multi-turn dialogue, task decomposition, and context-aware decision-making~\cite{}. Leveraging these capabilities, LLM-based agents are now being applied to complex, interactive tasks such as conversational assistance~\cite{}, tool-augmented reasoning~\cite{}, and autonomous decision-making in partially observable environments~\cite{}.
These applications generate extended interaction histories, which expose the limitations of fixed-length context windows.

Rather than relying on computationally expensive context window extensions~\cite{}, recent research has turned to external memory mechanisms to efficiently manage long-term context. These memory-augmented agents typically model memory as an external storage module, using retrieval methods to query relevant history and effectively expand their functional context window for long-horizon reasoning~\cite{}.  Considerable focus has been placed on sophisticated storage mechanisms. For instance, MemGPT~\cite{memgpt} introduces OS-inspired memory management and external paging, while Memory OS~\cite{memoryos} of AI Agent further modularizes memory ingestion, organization, and lifecycle management. These efforts highlight the importance of systematic abstractions, but they often remain tied to static orchestration rules. MemoryBank~\cite{memorybank} maintains a memory bank with write/retrieve/reflect cycles and relevance-aware updates. A-MEM~\cite{amem} formalizes pipelines for long-horizon agentic memory, while Mem0~\cite{mem0} emphasizes production-ready, scalable schemas. Alternative perspectives include Zep~\cite{zep}, which encodes context as a temporal knowledge graph to make temporal relations explicit, and Multiple Memory Systems~\cite{multiplememory}, which emulate human episodic vs. semantic divisions to enhance durability and transfer. However, despite these advances in memory storage, the querying of historical data often remains simplistic, typically relying on single-round, similarity-based search (e.g., BM25, dense retrieval). While Memory-R1~\cite{memoryr1} advances this by using reinforcement learning to optimize storage and retrieval policies, its retrieval is still a single-round process. To address this gap, our work, Agentic-Mem, introduces a Research Agent that handles complex queries through an iterative process of retrieval, reflection, and synthesis.


% Studies on memory for LLM-based agents generally converge on two essential questions: how to organize and compress long-horizon contexts and how to retrieve them efficiently at inference time.
% Several works conceptualize memory as an operating-system-like substrate. MemGPT~\cite{memgpt} introduces OS-inspired memory management and external paging, while Memory OS~\cite{memoryos} of AI Agent further modularizes memory ingestion, organization, and lifecycle management. These efforts highlight the importance of systematic abstractions, but they often remain tied to static orchestration rules.
% Other studies focus on structuring long-term contexts into lightweight representations. MemoryBank~\cite{memorybank} maintains a memory bank with write/retrieve/reflect cycles and relevance-aware updates. A-MEM~\cite{amem} formalizes pipelines for long-horizon agentic memory, while Mem0~\cite{mem0} emphasizes production-ready, scalable schemas. Alternative perspectives include Zep~\cite{zep}, which encodes context as a temporal knowledge graph to make temporal relations explicit, and Multiple Memory Systems~\cite{multiplememory}, which emulate human episodic vs. semantic divisions to enhance durability and transfer. While effective, these designs rely heavily on manual schema engineering and task-specific heuristics, limiting adaptability across domains.
% On the retrieval side, most frameworks combine sparse (BM25) and dense (embedding-based) search with lightweight re-ranking. Memory-R1~\cite{memoryr1} advances this line by introducing reinforcement learning to optimize what to store, when to evict, and how to query, thus closing the loop between storage policy and retrieval effectiveness. However, retrieval remains largely search-centric: queries return isolated snippets, but agents rarely engage in planning, multi-hop exploration, or evidence synthesis across raw and structured memory.
% Therefore, designing a new paradigm for general agentic memory that emphasizes flexibility, scalability, and minimal manual engineering remains a crucial challenge.


\paragraph{Retrieval-Augmented Generation for LLMs}.
Retrieval-Augmented Generation (RAG) enhances Large Language Models by grounding them in external knowledge sources~\cite{}. The standard paradigm involves chunking and indexing documents, retrieving relevant passages via semantic similarity, and using this context to augment the LLM's prompt~\cite{}. Subsequent advances have introduced sophisticated pre- and post-retrieval optimizations~\cite{}, culminating in agentic RAG systems. These systems exhibit autonomous retrieval behaviors, such as dynamically determining when and what to retrieve~\cite{}, generating hypothetical responses to guide search, and iteratively refining their strategies based on intermediate results~\cite{}.
Although agentic RAG demonstrates significant agency in the retrieval process, its objective remains to query a static knowledge base to optimize a single response. This stands in fundamental contrast to our agentic memory system. Our focus is on the autonomous management of dynamic historical context—automatically storing and updating memories and their relationships, and generating accurate summaries and guidance for current tasks according to the historical interactions through iterative reflection and synthesis.


==> table/main_newbench.tex <==
\begin{table*}[htbp]
\centering
\caption{Main results}
\label{tab:main}
\vspace{3pt}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{cl|cccccccc}
\hline
\multicolumn{1}{c}{\textbf{Model}} &
\multicolumn{1}{l|}{\textbf{Method}} &
\textbf{AIME} &
\textbf{GAIA} &
\textbf{HLE} &
\textbf{WebArena} &
\textbf{BrowseComp} &
\textbf{Tau-bench} &
\textbf{LiveCodeBench} &
\textbf{Average} \\ \hline

% \multicolumn{2}{c|}{GPT-5} & 98.85 & 65.99 & 55.78 &  &  &  & 49.66 &  \\ 
% \multicolumn{2}{c|}{GPT-4o-mini} & 86.21 & 57.82 & 55.78 &  &  &  & 48.30 &  \\ 
% \multicolumn{2}{c|}{Qwen2.5 14b} & 89.66 & 63.27 & 51.02 &  &  &  & 45.58 &  \\ \hline

\multirow{6}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
& \textsc{RAG}         & 79.31 & 54.42 & 36.73 &  &  & 32.95 & 41.84 &  \\
& \textsc{A-mem}      & 62.07 & 53.06 & 44.90 &  &  & 12.24 & 32.46 &  \\
& \textsc{Mem0}       & 52.87 & 39.46 & 26.50 &  &  & 14.41 & 24.68 &  \\
& \textsc{MemoryOS}   & 57.47 & 34.01 & 32.48 &  &  & 26.26 & 27.31 &  \\
& \textsc{LightMem}    &  &  &  &  &  &  &  &  \\
& \textsc{GAM}         &  &  &  &  &  &  &  &  \\  \hline

\multirow{6}{*}{\textbf{\rotatebox{90}{Qwen2.5 14b}}}
& \textsc{RAG}         & 74.71 & 55.10 & 38.78 &  &  & 34.66 & 38.78 &  \\
& \textsc{A-mem}      & 62.07 & 46.94 & 40.82 &  &  & 10.71 & 28.71 &  \\
& \textsc{Mem0}       & 48.28 & 36.05 & 27.64 &  &  & 12.67 & 22.59 &  \\
& \textsc{MemoryOS}   & 50.57 & 29.93 & 21.77 &  &  & 13.84 & 23.52 &  \\
& \textsc{LightMem}    &  &  &  &  &  &  &  &  \\
& \textsc{GAM}         &  &  &  &  &  &  &  &  \\  \hline

\end{tabular}%
}
\end{table*}


==> table/main_results.tex <==
% \begin{table*}[htbp]
% \centering
% \caption{Main results}
% \label{tab:main}
% \vspace{3pt}
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{cl|cccccccc|c|cc|cc}
% \hline
% \multicolumn{1}{c}{\textbf{Model}} &
% \multicolumn{1}{l|}{\textbf{Method}} &
% \multicolumn{8}{c|}{\textbf{LoCoMo}} &
% \multicolumn{1}{c|}{\textbf{HotpotQA}} &
% \multicolumn{2}{c|}{\textbf{LongBench v2}} &
% \multicolumn{2}{c}{\textbf{LongCodeBench}} \\ \cline{3-15}
% & & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} &
% \multicolumn{1}{c|}{} &
% \textbf{Easy} & \textbf{Hard} &
% \textbf{256k} & \textbf{512k} \\
% & & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} &
% \textbf{F1} &
% \textbf{Acc.} & \textbf{Acc.} &
% \textbf{Acc.} & \textbf{Acc.} \\ \hline

% \hline

% \multirow{8}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
% & \textsc{RAG}         & \underline{52.45} & \underline{47.94} & 27.50 & 20.13 & 46.07 & 40.35 & 23.23 & 17.94 & 68.56 & 33.85 & 28.30 & 53.85 & 57.45 \\
% & \textsc{A-mem}       & 44.65 & 37.06 & 27.02 & 20.09 & 45.85 & 36.67 & 12.14 & 12.00 & - & - & - & - & - \\
% & \textsc{A-mem*}      & 34.02 & 27.73 & 21.77 & 16.65 & 35.13 & 30.74 & 10.79 & 9.89 & 66.82 & 32.81 & 27.65 & 63.08 & 68.09 \\
% & \textsc{Mem0}        & 47.65 & 38.72 & \underline{38.72} & 27.13 & \underline{48.93} & \underline{40.51} & \textbf{28.64} & \underline{21.58} & - & - & - & - & - \\
% & \textsc{Mem0*}       & 36.63 & 32.13 & 24.66 & 18.04 & 38.42 & 33.64 & 14.19 & 10.62 & 72.48 & 29.69 & 25.40 & 61.54 & \underline{70.21} \\
% & \textsc{MemoryOS}    & 48.62 & 42.99 & 35.27 & 25.22 & 41.15 & 30.76 & 20.02 & 16.52 & - & - & - & - & - \\
% & \textsc{MemoryOS*}   & 44.16 & 38.42 & 36.58 & \underline{28.79} & 35.24 & 26.54 & 22.72 & 16.65 & \underline{74.37} & \underline{35.42} & \underline{30.23} & \underline{64.62} & 68.09 \\
% & \textsc{LightMem*}    &  &  &  &  &  &  &  &  &  &  &  &  &  \\


% & \textsc{GAM}        & \textbf{58.13} & \textbf{52.54} & \textbf{40.64} & \textbf{32.17} & \textbf{56.16} & \textbf{49.86} & \underline{27.58} & \textbf{21.95} & \textbf{77.26} & \textbf{40.63} & \textbf{37.30} & \textbf{69.23} & \textbf{74.46} \\ \hline

% \multirow{5}{*}{\textbf{\rotatebox{90}{Qwen2.5 14b}}}
% & \textsc{RAG}      & \underline{47.87} & \underline{42.79} & 26.38 & 19.54 & 30.78 & 25.97 & 14.16 & 10.52 & 64.67 & \underline{35.42} & \textbf{34.41} & 55.38 & 61.70 \\
% & \textsc{A-mem*}      & 33.75 & 30.04 & 22.09 & 15.28 & 27.19 & 22.05 & 13.49 & 10.74 & 63.53 & 31.77 & \underline{28.62} & \textbf{66.15} & \textbf{68.09} \\
% & \textsc{Mem0*}       & 42.58 & 35.15 & 31.73 & 24.82 & 28.96 & 26.24 & 15.03 & 11.28 & 65.60 & 30.21 & 27.97 & 61.54 & \underline{65.96} \\
% & \textsc{MemoryOS*}    & 46.33 & 41.62 & \underline{38.19} & \underline{29.26} & \underline{32.24} & \underline{27.86} & \underline{20.27} & \underline{15.94} & \textbf{75.42} & 33.85 & 26.69 & 63.08 & 63.83 \\
% & \textsc{LightMem*}    &  &  &  &  &  &  &  &  &  &  &  &  &  \\

% & \textsc{GAM}        & \textbf{54.26} & \textbf{49.14}& \textbf{41.54} & \textbf{33.63} & \textbf{48.33} & \textbf{42.91} & \textbf{27.97} & \textbf{22.67} & \underline{74.18} & \textbf{36.98} & \textbf{34.41} & \underline{64.62} & \textbf{68.09}  \\ \hline

% \end{tabular}%
% }
% \end{table*}


\begin{table*}[htbp]
\centering
\caption{Main results}
\label{tab:main}
\vspace{3pt}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{cl|cccccccc|c|c|cc}
\hline
\multicolumn{1}{c}{\textbf{Model}} &
\multicolumn{1}{l|}{\textbf{Method}} &
\multicolumn{8}{c|}{\textbf{LoCoMo}} &
\multicolumn{1}{c|}{\textbf{LongBenchv2}} &
\multicolumn{1}{c|}{\textbf{LongMemEval}} &
\multicolumn{2}{c}{\textbf{LongCodeBench}} \\ \cline{3-14}
& & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} & & &
\textbf{256k} & \textbf{512k} \\
& & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{Acc.} & \textbf{BLEU-1} &
\textbf{F1} &
\textbf{Acc.} &
\textbf{Acc.} & \textbf{Acc.} \\ \hline

% \hline

% \multirow{9}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
% & \textsc{RAG}         & \underline{52.45} & \underline{47.94} & 27.50 & 20.13 & 46.07 & 40.35 & 23.23 & 17.94 & 68.56 & 55.20 & 53.85 & 57.45 \\
% & \textsc{A-mem}       & 44.65 & 37.06 & 27.02 & 20.09 & 45.85 & 36.67 & 12.14 & 12.00 & - & - & - & - \\
% & \textsc{A-mem*}      & 34.02 & 27.73 & 21.77 & 16.65 & 35.13 & 30.74 & 10.79 & 9.89 & 66.82 & 61.20 & 63.08 & 68.09 \\
% & \textsc{Mem0}        & 47.65 & 38.72 & \underline{38.72} & 27.13 & \underline{48.93} & \underline{40.51} & \underline{28.64} & \underline{21.58} & - & - & - & - \\
% & \textsc{Mem0*}       & 36.63 & 32.13 & 24.66 & 18.04 & 38.42 & 33.64 & 14.19 & 10.62 & 72.48 & 49.40 & 61.54 & \underline{70.21} \\
% & \textsc{MemoryOS}    & 48.62 & 42.99 & 35.27 & 25.22 & 41.15 & 30.76 & 20.02 & 16.52 & - & - & - & - \\
% & \textsc{MemoryOS*}   & 44.16 & 38.42 & 36.58 & \underline{28.79} & 35.24 & 26.54 & 22.72 & 16.65 & \textbf{74.37} & 51.80 & 64.62 & 68.09 \\
% & \textsc{LightMem*}   & 41.79 & 37.83 & 29.78 & 24.80 & 43.71 & 39.72 & 16.89 & 13.92 & 69.51 & \underline{65.40} & \underline{66.15} & \underline{70.21} \\

% & \textsc{GAM w/o memory}         &  &  &  &  &  &  &  &  &  &  & &  \\

% & \textsc{GAM w. memory}        & \textbf{56.62} & \textbf{51.36} & \textbf{41.13} & \textbf{33.08} & \textbf{56.15} & \textbf{49.82} & \textbf{30.79} & \textbf{24.65} & \underline{73.59} & \textbf{67.20} & \textbf{69.23} & \textbf{72.34} \\ \hline


\multirow{7}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
& \textsc{w/o memory}         &  &  &  &  &  &  &  &  &  &  & &  \\
& \textsc{RAG}         & \underline{52.45} & \underline{47.94} & 27.50 & 20.13 & 46.07 & 40.35 & 23.23 & 17.94 & 68.56 & 55.20 & 53.85 & 57.45 \\
& \textsc{A-mem}       & 44.65 & 37.06 & 27.02 & 20.09 & 45.85 & 36.67 & 12.14 & 12.00 & 66.82 & 61.20 & 63.08 & 68.09 \\
& \textsc{Mem0}        & 47.65 & 38.72 & \underline{38.72} & 27.13 & \underline{48.93} & \underline{40.51} & \underline{28.64} & \underline{21.58} & 72.48 & 49.40 & 61.54 & \underline{70.21} \\
& \textsc{MemoryOS}    & 48.62 & 42.99 & 35.27 & 25.22 & 41.15 & 30.76 & 20.02 & 16.52 & \textbf{74.37} & 51.80 & 64.62 & 68.09 \\
& \textsc{LightMem}   & 41.79 & 37.83 & 29.78 & 24.80 & 43.71 & 39.72 & 16.89 & 13.92 & 69.51 & \textbf{68.64} & \underline{66.15} & \underline{70.21} \\

& \textsc{GAM}        & \textbf{56.62} & \textbf{51.36} & \textbf{41.13} & \textbf{33.08} & \textbf{56.15} & \textbf{49.82} & \textbf{30.79} & \textbf{24.65} & \underline{73.59} & \underline{67.20} & \textbf{69.23} & \textbf{72.34} \\ \hline



\multirow{7}{*}{\textbf{\rotatebox{90}{Qwen2.5 14b}}}
& \textsc{w/o memory}         &  &  &  &  &  &  &  &  &  &  & &  \\
& \textsc{RAG}         & \underline{47.87} & \underline{42.79} & 26.38 & 19.54 & 30.78 & 25.97 & 14.16 & 10.52 & 64.67 & 52.60 & 55.38 & 61.70 \\
& \textsc{A-mem}      & 33.75 & 30.04 & 22.09 & 15.28 & 27.19 & 22.05 & 13.49 & 10.74 & 63.53 & 57.20 & \textbf{66.15} & \textbf{68.09} \\
& \textsc{Mem0}       & 42.58 & 35.15 & 31.73 & 24.82 & 28.96 & 26.24 & 15.03 & 11.28 & 65.60 & 46.60 & 61.54 & \underline{65.96} \\
& \textsc{MemoryOS}   & 46.33 & 41.62 & \underline{38.19} & \underline{29.26} & \underline{32.24} & \underline{27.86} & \underline{20.27} & \underline{15.94} & \underline{71.34} & 54.40 & 63.08 & 63.83 \\
& \textsc{LightMem}   & 34.92 & 31.22 & 25.45 & 19.61 & 32.03 & 27.70 & 15.81 & 11.81 & 66.73 & \underline{58.20} & 61.54 & 63.83 \\


& \textsc{GAM}         & \textbf{57.09} & \textbf{51.62} & \textbf{42.55} & \textbf{34.98} & \textbf{40.96} & \textbf{35.09} & \textbf{24.27} & \textbf{19.23} & \textbf{72.25} & \textbf{61.80} & \underline{64.62} & \textbf{68.09} \\ \hline

\end{tabular}%
}
\end{table*}


==> table/main_results_update.tex <==
% \begin{table*}[htbp]
% \centering
% \caption{Main results}
% \label{tab:main}
% \vspace{3pt}
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{cl|cccccccc|ccc|c}
% \hline
% \multicolumn{1}{c}{\textbf{Model}} &
% \multicolumn{1}{l|}{\textbf{Method}} &
% \multicolumn{8}{c|}{\textbf{LoCoMo}} &
% \multicolumn{3}{c|}{\textbf{LongBench v2}} &
% \multicolumn{1}{c}{\textbf{LME}} \\ \cline{3-14}
% & & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} &
% \textbf{Short} & \textbf{Medium} & \textbf{Long} &
%  \\
% & & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} &
% \textbf{Acc.} & \textbf{Acc.} & \textbf{Acc.} & \textbf{Acc.} \\ \hline


% \multirow{7}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
% & \textsc{w/o memory}         & 46.68 & 37.54 & 29.23 & 22.76 & 25.97 & 19.42 & 16.87 & 13.70 & 32.78 & 28.37 & 24.07 & 54.80 \\
% & \textsc{RAG}         & \underline{52.45} & \underline{47.94} & 27.50 & 20.13 & 46.07 & 40.35 & 23.23 & 17.94 & 34.44 & 27.44 & 29.63 & 55.20 \\
% & \textsc{A-mem}       & 44.65 & 37.06 & 27.02 & 20.09 & 45.85 & 36.67 & 12.14 & 12.00 & 31.11 & 23.26 & 18.52 & 61.20 \\
% & \textsc{Mem0}        & 47.65 & 38.72 & \underline{38.72} & 27.13 & \underline{48.93} & \underline{40.51} & \underline{28.64} & \underline{21.58} & 27.78 & 18.14 & 12.03 & 49.40 \\
% & \textsc{MemoryOS}    & 48.62 & 42.99 & 35.27 & 25.22 & 41.15 & 30.76 & 20.02 & 16.52 & 36.67 & 21.39 & 20.37 & 51.80 \\
% & \textsc{LightMem}    & 41.79 & 37.83 & 29.78 & 24.80 & 43.71 & 39.72 & 16.89 & 13.92 & 26.67 & 17.67 & 19.44 & \textbf{68.64} \\
% & \textsc{GAM}         & \textbf{56.62} & \textbf{51.36} & \textbf{41.13} & \textbf{33.08} & \textbf{56.15} & \textbf{49.82} & \textbf{30.79} & \textbf{24.65} &  &  &  & \underline{67.20} \\ \hline

% \multirow{7}{*}{\textbf{\rotatebox{90}{Qwen2.5 14b}}}
% & \textsc{w/o memory}        & 46.05 & 39.56 & 32.08 & 24.46 & 30.51 & 24.45 & 14.89 & 11.41 & 35.56 & 29.77 & 24.07 & 37.20 \\
% & \textsc{RAG}         & \underline{47.87} & \underline{42.79} & 26.38 & 19.54 & 30.78 & 25.97 & 14.16 & 10.52 & 40.00 & 32.09 & 28.70 & 52.60 \\
% & \textsc{A-mem}       & 33.75 & 30.04 & 22.09 & 15.28 & 27.19 & 22.05 & 13.49 & 10.74 & 34.44 & 22.79 & 22.22 & 57.20 \\
% & \textsc{Mem0}        & 42.58 & 35.15 & 31.73 & 24.82 & 28.96 & 26.24 & 15.03 & 11.28 & 31.67 & 17.21 & 16.67 & 46.60 \\
% & \textsc{MemoryOS}    & 46.33 & 41.62 & \underline{38.19} & \underline{29.26} & \underline{32.24} & \underline{27.86} & \underline{20.27} & \underline{15.94} & 38.89 & 31.16 & 27.78 & 54.40 \\
% & \textsc{LightMem}    & 34.92 & 31.22 & 25.45 & 19.61 & 32.03 & 27.70 & 15.81 & 11.81 & 28.33 & 18.60 & 17.59 & \underline{58.20} \\
% & \textsc{GAM}         & \textbf{57.09} & \textbf{51.62} & \textbf{42.55} & \textbf{34.98} & \textbf{40.96} & \textbf{35.09} & \textbf{24.27} & \textbf{19.23} &  &  &  & \textbf{65.00} \\ \hline

% \end{tabular}%
% }
% \end{table*}


% \begin{table*}[htbp]
% \centering
% \caption{Main results}
% \label{tab:main}
% \vspace{3pt}
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{cl|cccccccc|ccc|ccc|c}
% \hline
% \multicolumn{1}{c}{\textbf{Model}} &
% \multicolumn{1}{l|}{\textbf{Method}} &
% \multicolumn{8}{c|}{\textbf{LoCoMo}} &
% \multicolumn{3}{c|}{\textbf{LongBench v2}} &
% \multicolumn{3}{c|}{\textbf{HotpotQA}} &
% \multicolumn{1}{c}{\textbf{LME}} \\ \cline{3-17}
% & & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} &
% \textbf{Short} & \textbf{Medium} & \textbf{Long} &
% \textbf{56K} & \textbf{224K} & \textbf{448K} & \\ 
% & & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{Acc.} & \textbf{Acc.} & \textbf{Acc.}  & \textbf{F1} & \textbf{F1} & \textbf{F1} & \textbf{Acc.}  \\ 

% \hline


% \multirow{7}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
% & \textsc{w/o memory}         & 46.68 & 37.54 & 29.23 & 22.76 & 25.97 & 19.42 & 16.87 & 13.70 & 32.78 & 28.37 & 24.07 &  &  &  & 54.80 \\
% & \textsc{RAG}         & \underline{52.45} & \underline{47.94} & 27.50 & 20.13 & 46.07 & 40.35 & 23.23 & 17.94 & 34.44 & 27.44 & 29.63 &  &  &  & 55.20 \\
% & \textsc{A-mem}       & 44.65 & 37.06 & 27.02 & 20.09 & 45.85 & 36.67 & 12.14 & 12.00 & 31.11 & 23.26 & 18.52 &  &  &  & 61.20 \\
% & \textsc{Mem0}        & 47.65 & 38.72 & \underline{38.72} & 27.13 & \underline{48.93} & \underline{40.51} & \underline{28.64} & \underline{21.58} & 27.78 & 18.14 & 12.03 &  &  &  & 49.40 \\
% & \textsc{MemoryOS}    & 48.62 & 42.99 & 35.27 & 25.22 & 41.15 & 30.76 & 20.02 & 16.52 & 36.67 & 21.39 & 20.37 &  &  &  & 51.80 \\
% & \textsc{LightMem}    & 41.79 & 37.83 & 29.78 & 24.80 & 43.71 & 39.72 & 16.89 & 13.92 & 26.67 & 17.67 & 19.44 &  &  &  & \textbf{68.64} \\
% & \textsc{GAM}         & \textbf{56.62} & \textbf{51.36} & \textbf{41.13} & \textbf{33.08} & \textbf{56.15} & \textbf{49.82} & \textbf{30.79} & \textbf{24.65} &  &  &  &  &  &  &  \\ \hline

% \multirow{7}{*}{\textbf{\rotatebox{90}{Qwen2.5 14b}}}
% & \textsc{w/o memory}        & 46.05 & 39.56 & 32.08 & 24.46 & 30.51 & 24.45 & 14.89 & 11.41 & 35.56 & 29.77 & 24.07 & 49.81 & 46.97 & 43.47 & 37.20 \\
% & \textsc{RAG}         & \underline{47.87} & \underline{42.79} & 26.38 & 19.54 & 30.78 & 25.97 & 14.16 & 10.52 & 40.00 & 32.09 & 28.70 & 51.83 & 46.91 & 48.34 & 52.60 \\
% & \textsc{A-mem}       & 33.75 & 30.04 & 22.09 & 15.28 & 27.19 & 22.05 & 13.49 & 10.74 & 34.44 & 22.79 & 22.22 & 27.48 & 26.08 &  & 57.20 \\
% & \textsc{Mem0}        & 42.58 & 35.15 & 31.73 & 24.82 & 28.96 & 26.24 & 15.03 & 11.28 & 31.67 & 17.21 & 16.67 &  &  &  & 46.60 \\
% & \textsc{MemoryOS}    & 46.33 & 41.62 & \underline{38.19} & \underline{29.26} & \underline{32.24} & \underline{27.86} & \underline{20.27} & \underline{15.94} & 38.89 & 31.16 & 27.78 & 24.41 & 19.85 &  & 54.40 \\
% & \textsc{LightMem}    & 34.92 & 31.22 & 25.45 & 19.61 & 32.03 & 27.70 & 15.81 & 11.81 & 28.33 & 18.60 & 17.59 &  &  &  & \underline{58.20} \\
% & \textsc{GAM}         & \textbf{57.09} & \textbf{51.62} & \textbf{42.55} & \textbf{34.98} & \textbf{40.96} & \textbf{35.09} & \textbf{24.27} & \textbf{19.23} &  &  &  &  63.75 & 55.86 & 57.76 &  \\ \hline

% \end{tabular}%
% }
% \end{table*}






% \begin{table*}[htbp]
% \centering
% \caption{Main results}
% \label{tab:main}
% \vspace{3pt}
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{cl|cccccccc|ccc|c}
% \hline
% \multicolumn{1}{c}{\textbf{Model}} &
% \multicolumn{1}{l|}{\textbf{Method}} &
% \multicolumn{8}{c|}{\textbf{LoCoMo}} &
% \multicolumn{3}{c|}{\textbf{HotpotQA}} &
% \multicolumn{1}{c}{\textbf{LME}} \\ \cline{3-14}
% & & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} &
% \textbf{56K} & \textbf{224K} & \textbf{448K} & \textbf{Acc.}  \\ 
% & & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{F1} & \textbf{F1} & \textbf{Acc.}  \\ 

% \hline

% \multirow{7}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
% & \textsc{w/o memory}         & 46.68 & 37.54 & 29.23 & 22.76 & 25.97 & 19.42 & 16.87 & 13.70 &  &  &  & 54.80 \\
% & \textsc{RAG}         & \underline{52.45} & \underline{47.94} & 27.50 & 20.13 & 46.07 & 40.35 & 23.23 & 17.94 &  &  &  & 55.20 \\
% & \textsc{A-mem}       & 44.65 & 37.06 & 27.02 & 20.09 & 45.85 & 36.67 & 12.14 & 12.00 &  &  &  & 61.20 \\
% & \textsc{Mem0}        & 47.65 & 38.72 & \underline{38.72} & 27.13 & \underline{48.93} & \underline{40.51} & \underline{28.64} & \underline{21.58} &  &  &  & 49.40 \\
% & \textsc{MemoryOS}    & 48.62 & 42.99 & 35.27 & 25.22 & 41.15 & 30.76 & 20.02 & 16.52 &  &  &  & 51.80 \\
% & \textsc{LightMem}    & 41.79 & 37.83 & 29.78 & 24.80 & 43.71 & 39.72 & 16.89 & 13.92 &  &  &  & \textbf{68.64} \\
% & \textsc{GAM}         & \textbf{56.62} & \textbf{51.36} & \textbf{41.13} & \textbf{33.08} & \textbf{56.15} & \textbf{49.82} & \textbf{30.79} & \textbf{24.65} &  &  &  &  \\ \hline

% \multirow{7}{*}{\textbf{\rotatebox{90}{Qwen2.5 14b}}}
% & \textsc{w/o memory}        & 46.05 & 39.56 & 32.08 & 24.46 & 30.51 & 24.45 & 14.89 & 11.41 & 49.81 & 46.97 & 43.47 & 37.20 \\
% & \textsc{RAG}         & \underline{47.87} & \underline{42.79} & 26.38 & 19.54 & 30.78 & 25.97 & 14.16 & 10.52 & 51.83 & 46.91 & 48.34 & 52.60 \\
% & \textsc{A-mem}       & 33.75 & 30.04 & 22.09 & 15.28 & 27.19 & 22.05 & 13.49 & 10.74 & 27.48 & 26.08 &  & 57.20 \\
% & \textsc{Mem0}        & 42.58 & 35.15 & 31.73 & 24.82 & 28.96 & 26.24 & 15.03 & 11.28 &  &  &  & 46.60 \\
% & \textsc{MemoryOS}    & 46.33 & 41.62 & \underline{38.19} & \underline{29.26} & \underline{32.24} & \underline{27.86} & \underline{20.27} & \underline{15.94} & 24.41 & 19.85 &  & 54.40 \\
% & \textsc{LightMem}    & 34.92 & 31.22 & 25.45 & 19.61 & 32.03 & 27.70 & 15.81 & 11.81 &  &  &  & \underline{58.20} \\
% & \textsc{GAM}         & \textbf{57.09} & \textbf{51.62} & \textbf{42.55} & \textbf{34.98} & \textbf{40.96} & \textbf{35.09} & \textbf{24.27} & \textbf{19.23} & \textbf{63.75} & \textbf{55.86} & \textbf{57.76} & \textbf{65.00} \\ \hline

% \end{tabular}%
% }
% \end{table*}





% \begin{table*}[htbp]
% \centering
% \caption{Main results}
% \label{tab:main}
% \vspace{3pt}
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{cl|cccccccc|ccc|cccc|c}
% \hline
% \multicolumn{1}{c}{\textbf{Model}} &
% \multicolumn{1}{l|}{\textbf{Method}} &
% \multicolumn{8}{c|}{\textbf{LoCoMo}} &
% \multicolumn{3}{c|}{\textbf{HotpotQA}} &
% \multicolumn{4}{c|}{\textbf{RULER(128k)}} &

% \multicolumn{1}{c|}{\textbf{NarrativeQA}} \\ \cline{3-18}
% & & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} &
% \textbf{56K} & \textbf{224K} & \textbf{448K} & \textbf{Retri.} & \textbf{MT} & \textbf{Aggre} & \textbf{QA} &  \\ 
% & & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{F1} & \textbf{F1} & \textbf{Acc.} &\textbf{Acc.} &\textbf{Acc.} & \textbf{Acc.} & \textbf{F1}  \\ 
% \hline

% \multirow{7}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
% & \textsc{w/o memory}         & 46.68 & 37.54 & 29.23 & 22.76 & 25.97 & 19.42 & 16.87 & 13.70 & 56.56 & 54.29 & 53.92 & 80.30 & 60.60 & 36.70 & 61.60 &  31.26  \\
% & \textsc{RAG}         & \underline{52.45} & \underline{47.94} & 27.50 & 20.13 & 46.07 & 40.35 & 23.23 & 17.94 & 52.71 & 51.84 & 54.01 & 94.25 & 0.00 & 35.50 & 55.90 & 25.00  \\
% & \textsc{A-mem}       & 44.65 & 37.06 & 27.02 & 20.09 & 45.85 & 36.67 & 12.14 & 12.00 & 33.90 & 30.22 & 31.37 & & & & & 27.07  \\
% & \textsc{Mem0}        & 47.65 & 38.72 & \underline{38.72} & 27.13 & \underline{48.93} & \underline{40.51} & \underline{28.64} & \underline{21.58} & 32.58 & 31.74 & 27.41 &  & &  & & \\
% & \textsc{MemoryOS}    & 48.62 & 42.99 & 35.27 & 25.22 & 41.15 & 30.76 & 20.02 & 16.52 & 26.47 & 23.10 & 24.16 & 63.10 & 2.40 & 35.60 & 36.90 & 26.70  \\
% & \textsc{LightMem}    & 41.79 & 37.83 & 29.78 & 24.80 & 43.71 & 39.72 & 16.89 & 13.92 & 40.93 & 35.28 &  & & & & &  \\
% & \textsc{GAM}         & \textbf{56.62} & \textbf{51.36} & \textbf{41.13} & \textbf{33.08} & \textbf{56.15} & \textbf{49.82} & \textbf{30.79} & \textbf{24.65} & 63.22 & 64.56 & 59.81 & 97.70 & 93.20 & 42.50 & 72.50 & 36.86  \\ \hline

% \multirow{7}{*}{\textbf{\rotatebox{90}{Qwen2.5 14b}}}
% & \textsc{w/o memory}        & 46.05 & 39.56 & 32.08 & 24.46 & 30.51 & 24.45 & 14.89 & 11.41 & 49.75 & 46.82 & 43.17 & 70.85 & 80.00  & 15.40 & 45.60 & 29.69  \\
% & \textsc{RAG}         & \underline{47.87} & \underline{42.79} & 26.38 & 19.54 & 30.78 & 25.97 & 14.16 & 10.52 & 51.81 & 46.72 & 48.36 & 92.78 & 0.00 & 24.70 & 47.80 & 18.29  \\
% & \textsc{A-mem}       & 33.75 & 30.04 & 22.09 & 15.28 & 27.19 & 22.05 & 13.49 & 10.74 & 27.04 & 25.65 & 22.92 & & & & &  25.18  \\
% & \textsc{Mem0}        & 42.58 & 35.15 & 31.73 & 24.82 & 28.96 & 26.24 & 15.03 & 11.28 & 30.12 & 32.44 & 26.55 & & & &  & 27.80  \\
% & \textsc{MemoryOS}    & 46.33 & 41.62 & \underline{38.19} & \underline{29.26} & \underline{32.24} & \underline{27.86} & \underline{20.27} & \underline{15.94} & 24.58 & 30.25 & 23.13 & 54.58 & 3.00 & 5.20 & 34.60 & 23.45  \\
% & \textsc{LightMem}    & 34.92 & 31.22 & 25.45 & 19.61 & 32.03 & 27.70 & 15.81 & 11.81 & 37.30 & 27.72 & 28.25 & 27.53 & 17.40 & 25.60 & 53.00 & 16.57  \\
% & \textsc{GAM}         & \textbf{58.93} & \textbf{53.74} & \textbf{42.96} & \textbf{34.48} & \textbf{51.52} & \textbf{44.43} & \textbf{30.63} & \textbf{26.04} & \textbf{64.07} & \textbf{55.99} & \textbf{57.87} & 93.43 & 90.20 & 36.10 & 74.50 & \textbf{34.77} \\ \hline

% \end{tabular}%
% }
% \end{table*}

\begin{table*}[htbp]
\centering
\caption{Main results with Avg}
\label{tab:main}
\vspace{3pt}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{cl|cccccccc|ccc|cccc|c|c}
\hline
\multicolumn{1}{c}{\textbf{Model}} &
\multicolumn{1}{l|}{\textbf{Method}} &
\multicolumn{8}{c|}{\textbf{LoCoMo}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\multicolumn{4}{c|}{\textbf{RULER(128k)}} &
\multicolumn{1}{c|}{\textbf{NarrativeQA}} &
\multicolumn{1}{c}{\textbf{Avg}} \\ \cline{3-19}
& & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} &
\textbf{56K} & \textbf{224K} & \textbf{448K} & \textbf{Retri.} & \textbf{MT} & \textbf{Aggre} & \textbf{QA} & \textbf{F1} \\ 
& & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{F1} & \textbf{F1} & \textbf{Acc.} & \textbf{Acc.} & \textbf{Acc.} & \textbf{Acc.} & \textbf{F1} \\ 
\hline

\multirow{7}{*}{\textbf{\rotatebox{90}{GPT-4o-mini}}}
& \textsc{w/o memory}         & 46.68 & 37.54 & 29.23 & 22.76 & 25.97 & 19.42 & 16.87 & 13.70 & 56.56 & 54.29 & 53.92 & 80.30 & 60.60 & 36.70 & 61.60 & 31.26 & 40.46 \\
& \textsc{RAG}                & \underline{52.45} & \underline{47.94} & 27.50 & 20.13 & 46.07 & 40.35 & 23.23 & 17.94 & 52.71 & 51.84 & 54.01 & 94.25 & 0.00 & 35.50 & 55.90 & 25.00 & 40.30 \\
& \textsc{A-mem}              & 44.65 & 37.06 & 27.02 & 20.09 & 45.85 & 36.67 & 12.14 & 12.00 & 33.90 & 30.22 & 31.37 & - & - & - & - & 27.07 & - \\
& \textsc{Mem0}               & 47.65 & 38.72 & \underline{38.72} & \underline{27.13} & \underline{48.93} & \underline{40.51} & \underline{28.64} & \underline{21.58} & 32.58 & 31.74 & 27.41 & - & - & - & - & - & - \\
& \textsc{MemoryOS}           & 48.62 & 42.99 & 35.27 & 25.22 & 41.15 & 30.76 & 20.02 & 16.52 & 26.47 & 23.10 & 24.16 & 63.10 & 2.40 & 35.60 & 36.90 & 26.70 & 31.19 \\
& \textsc{LightMem}           & 41.79 & 37.83 & 29.78 & 24.80 & 43.71 & 39.72 & 16.89 & 13.92 & 40.93 & 35.28 & 30.02 & - & 36.20 & - & 52.60 & 17.51 & - \\
& \textsc{GAM}                & \textbf{56.62} & \textbf{51.36} & \textbf{41.13} & \textbf{33.08} & \textbf{56.15} & \textbf{49.82} & \textbf{30.79} & \textbf{24.65} & \textbf{63.22} & \textbf{64.56} & \textbf{59.81} & \textbf{97.70} & \textbf{93.20} & \textbf{42.50} & \textbf{72.50} & \textbf{36.86} & \textbf{54.62} \\ \hline

\multirow{7}{*}{\textbf{\rotatebox{90}{Qwen2.5 14b}}}
& \textsc{w/o memory}         & 46.05 & 39.56 & 32.08 & 24.46 & 30.51 & 24.45 & 14.89 & 11.41 & 49.75 & 46.82 & 43.17 & 70.85 & 80.00 & 15.40 & 45.60 & 29.69 & 37.79 \\
& \textsc{RAG}                & 47.87 & 42.79 & 26.38 & 19.54 & 30.78 & 25.97 & 14.16 & 10.52 & 51.81 & 46.72 & 48.36 & 92.78 & 0.00 & 24.70 & 47.80 & 18.29 & 34.28 \\
& \textsc{A-mem}              & 33.75 & 30.04 & 22.09 & 15.28 & 27.19 & 22.05 & 13.49 & 10.74 & 27.04 & 25.65 & 22.92 & - & - & - & - & 25.18 & - \\
& \textsc{Mem0}               & 42.58 & 35.15 & 31.73 & 24.82 & 28.96 & 26.24 & 15.03 & 11.28 & 30.12 & 32.44 & 26.55 & - & - & - & - & 27.80 & - \\
& \textsc{MemoryOS}           & 46.33 & 41.62 & 38.19 & 29.26 & 32.24 & 27.86 & 20.27 & 15.94 & 24.58 & 30.25 & 23.13 & 54.58 & 3.00 & 5.20 & 34.60 & 23.45 & 28.16 \\
& \textsc{LightMem}           & 34.92 & 31.22 & 25.45 & 19.61 & 32.03 & 27.70 & 15.81 & 11.81 & 37.30 & 27.72 & 28.25 & 27.53 & 17.40 & 25.60 & 53.00 & 16.57 & 27.00 \\
& \textsc{GAM}                & 58.93 & 53.74 & 42.96 & 34.48 & 51.52 & 44.43 & 30.63 & 26.04 & 64.07 & 55.99 & 57.87 & 93.43 & 90.20 & 36.10 & 74.50 & 34.77 & 53.10 \\ \hline

\end{tabular}}
\end{table*}








\begin{table*}[htbp]
\centering
\caption{Performance of different backbone models as memory (left) and research (right) models.}
\label{tab:mem_research_models}
\vspace{3pt}

\begin{minipage}{0.48\textwidth}
\centering
\textbf{(a) Memory Model}\\[3pt]
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{3}{*}{\textbf{Model}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\
& \textbf{F1} & \textbf{F1} & \textbf{F1} & & \\
\hline
\textsc{Qwen2.5 0.5B}  & 56.46 & 55.96 & 53.33 & 29.55 & 48.83 \\
\textsc{Qwen2.5 3B}    & 58.05 & 56.52 & 55.50 & 32.10 & 50.54 \\
\textsc{Qwen2.5 7B}    & 59.06 & 58.34 & 56.17 & 32.53 & 51.53 \\
\textsc{Qwen2.5 14B}   & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\
\textsc{Qwen2.5 32B}   & 63.05 & 59.75 & 56.26 & 34.94 & 53.50 \\
\textsc{GPT-4o mini}   & 64.77 & 59.29 & 57.25 & 34.87 & 54.05 \\
\hline
\end{tabular}%
}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\textbf{(b) Research Model}\\[3pt]
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{3}{*}{\textbf{Model}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\
& \textbf{F1} & \textbf{F1} & \textbf{F1} & & \\
\hline
\textsc{Qwen2.5 0.5B}  & 10.03 & 11.14 & 11.64 & 3.50 & 9.08 \\
\textsc{Qwen2.5 3B}    & 39.76 & 37.16 & 33.04 & 23.96 & 33.48 \\
\textsc{Qwen2.5 7B}    & 51.95 & 47.95 & 48.55 & 26.93 & 43.85 \\
\textsc{Qwen2.5 14B}   & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\
\textsc{Qwen2.5 32B}   & 61.93 & 59.19 & 61.53 & 35.33 & 54.50 \\
\textsc{GPT-4o-mini}   & 62.06 & 62.97 & 61.54 & 35.24 & 55.45 \\
\hline
\end{tabular}%
}
\end{minipage}

\end{table*}



% \begin{table*}[htbp]
% \centering
% \caption{Memory Model}
% \label{tab:main}
% \vspace{3pt}
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{l|cccccccc|ccc|c}
% \hline
% \multirow{3}{*}{\textbf{Model}} &
% \multicolumn{8}{c|}{\textbf{LoCoMo}} &
% \multicolumn{3}{c|}{\textbf{HotpotQA}} &
% \textbf{NarrativeQA} \\ 
% \cline{2-13}
% & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} & \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} \\
% & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{F1} & \textbf{F1} & \\ 
% \hline

% \textsc{Qwen2.5 0.5B}  & 51.61 & 46.54 & 39.97 & 32.20 & 47.22 & 41.41 & 24.24 & 19.53 & 56.46 & 55.96 & 53.33 & 29.55 \\
% \textsc{Qwen2.5 3B}  & 55.08 & 49.69 & 42.79 & 34.75 & 50.40 & 43.64 & 27.76 & 23.17 & 55.47 & 56.52 & 53.12 & 32.10 \\
% \textsc{Qwen2.5 7B}  & 56.75 & 50.98 & 43.46 & 36.15 & 48.81 & 42.51 & 25.79 & 20.49 & 59.06 & 58.34 & 56.17 & 32.53 \\
% \textsc{Qwen2.5 14B}  & 58.93 & 53.74 & 42.96 & 34.48 & 51.42 & 44.43 & 30.63 & 26.04 & 64.07 & 55.99 & 57.87 &  34.77 \\
% \textsc{Qwen2.5 32B}  &  &  &  &  &  &  &  &  & 60.29 & 59.75 & 56.26 &      \\
% \textsc{Qwen2.5 72B}  &  &  &  &  &  &  &  &  & 58.09 & 60.82 & &   \\
% \textsc{Gemini-2.5-flash-lite} & 58.26 & 52.56 & 42.82 & 35.37 & 51.36 & 45.40 & 28.98 & 24.19 & & & & \\
% \hline
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[htbp]
\centering
\caption{Memory Model}
\label{tab:main_simplified}
\vspace{3pt}
\resizebox{0.8\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{3}{*}{\textbf{Model}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\ 
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\ 
& \textbf{F1} & \textbf{F1} & \textbf{F1} &  & \\ 
\hline

\textsc{Qwen2.5 0.5B}  & 56.46 & 55.96 & 53.33 & 29.55 & 48.83 \\
\textsc{Qwen2.5 3B}    & 58.05 & 56.52 & 55.50 & 32.10 & 50.54 \\
\textsc{Qwen2.5 7B}    & 59.06 & 58.34 & 56.17 & 32.53 & 51.53 \\
\textsc{Qwen2.5 14B}   & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\
\textsc{Qwen2.5 32B}   & 63.05 & 59.75 & 56.26 & 34.94 & 53.50 \\
\textsc{GPT-4o mini}   & 64.77 & 59.29 & 57.25 & 34.87 & 54.05 \\
\hline
\end{tabular}%
}
\end{table*}


% \begin{table*}[htbp]
% \centering
% \caption{Integration Result}
% \label{tab:main}
% \vspace{3pt}
% \resizebox{\textwidth}{!}{%
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{l|cccccccc|ccc|c}
% \hline
% \multirow{3}{*}{\textbf{Model}} &
% \multicolumn{8}{c|}{\textbf{LoCoMo}} &
% \multicolumn{3}{c|}{\textbf{HotpotQA}} &
% \textbf{NarrativeQA} \\ 
% \cline{2-13}
% & \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} & \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} \\
% & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{F1} & \textbf{F1} & \\ 
% \hline

% \textsc{Only Integration Result} & 58.93 & 53.74 & 42.96 & 34.48 & 51.42 & 44.43 & 30.63 & 26.04 & 64.07 & 55.99 & 57.87 & 34.77 \\
% \textsc{\quad w/ Page} & 60.81 & 55.02 & 45.05 & 37.06 & 53.61 & 46.49 & 24.25 & 21.26 & 62.97 & 60.40 & 59.42 & 34.05 \\
% \textsc{\quad w/ Extrated Content} & 59.05 & 53.36 & 42.92 & 35.27 & 50.94 & 44.98 & 28.92 & 24.19 & 65.69 & 57.83 & 57.81 & 35.57 \\

% \textsc{\quad w/ Page Only} &  &  &  &  &  &  &  &  & 11.12 & 9.98 & 14.95 & \\
% \textsc{\quad w/ Extrated Content Only} &  &  &  &  &  &  &  &  & 57.79 & 53.76 & 57.03 &\\

% \hline
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[htbp]
\centering
\caption{Integration Result}
\label{tab:main_simplified}
\vspace{3pt}
\resizebox{0.8\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\ 
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\ 
 & \textbf{F1} & \textbf{F1} & \textbf{F1} &  & \\
\hline

\textsc{Only Integration Result} & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\
\textsc{\quad w/ Page} & 62.97 & 60.40 & 59.42 & 34.05 & 54.21 \\
\textsc{\quad w/ Extrated Content} & 65.69 & 57.83 & 57.81 & 35.57 & 54.73 \\

% \textsc{\quad w/ Page Only} & 11.12 & 9.98 & 14.95 &  & 12.02 \\
% \textsc{\quad w/ Extrated Content Only} & 57.79 & 53.76 & 57.03 &  & 56.19 \\

\hline
\end{tabular}%
}
\end{table*}




\begin{table*}[htbp]
\centering
\caption{Reflection Depth}
\label{tab:main_simplified}
\vspace{3pt}
\resizebox{0.8\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{2}{*}{\textbf{Depth}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\ 
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\ 
 & \textbf{F1} & \textbf{F1} & \textbf{F1} &  & \\
\hline


\textsc{1} & 59.79 & 46.81 & 46.77 & 30.76 & 46.03 \\
\textsc{2} & 62.85 & 55.66 & 57.50 & 32.21 & 52.06 \\
\textsc{3} & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\
\textsc{4} & 64.96 & 60.48 & 60.26 & 34.96 & 55.17 \\
\textsc{5} & 66.15 & 61.42 & 61.23 & 35.13 & 55.98 \\


\hline
\end{tabular}%
}
\end{table*}







\begin{table*}[htbp]
\centering
\caption{Tools Impact}
\label{tab:tools}
\vspace{3pt}
\resizebox{0.8\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{2}{*}{\textbf{Tools}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\ 
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\ 
 & \textbf{F1} & \textbf{F1} & \textbf{F1} &  & \\
\hline

\textsc{Only Page-id} & 28.07 & 16.32 & 13.82 & 31.74 & 22.49 \\
\textsc{Only Embedding} & 38.57 & 31.38 & 27.09 & 32.08 & 32.28\\
\textsc{Only BM25} & 59.79 & 53.58 & 49.91 & 31.78 & 48.77 \\
\textsc{Embedding+Page-id} & 42.41 & 30.35 & 29.54 & 33.84 & 34.04 \\
\textsc{Embedding+BM25} & 63.19 & 55.91 & 55.94 & 33.21 & 52.06\\
\textsc{BM25+Page-id} & 63.52 & 55.29 & 55.93 & 33.50 & 52.06\\
\textsc{All} & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\
\hline
\end{tabular}%
}
\end{table*}



\begin{table*}[htbp]
\centering
\caption{Retrieval Pages}
\label{tab:main_simplified}
\vspace{3pt}
\resizebox{0.8\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{2}{*}{\textbf{Num of Pages}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\ 
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\ 
 & \textbf{F1} & \textbf{F1} & \textbf{F1} &  & \\
\hline

\textsc{3}  & 62.70 & 48.69 & 55.63 & 33.57 & 50.15 \\
\textsc{5}  & 64.07 & 55.99 & 57.87 & 34.77 & 53.18\\
\textsc{10} & 64.04 & 57.13 & 59.44 & 34.43 & 53.76\\
\textsc{20} & 65.72 & 60.50 & 61.29 & 34.92 & 55.61\\
\hline
\end{tabular}%
}
\end{table*}



\begin{table*}[htbp]
\centering
\caption{Ablation Study}
\label{tab:agents}
\vspace{3pt}
\resizebox{0.8\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\ 
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\ 
 & \textbf{F1} & \textbf{F1} & \textbf{F1} &  & \\
\hline
\textsc{full}  & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\
\textsc{w/o memory planning} & 57.40 & 49.72 & 53.98 & 31.97 & 48.27 \\
\textsc{w/o research agent} & 42.67 & 19.75 & 17.38 & 30.18 & 27.50 \\
\hline
\end{tabular}%
}
\end{table*}



\begin{table*}[htbp]
\centering
\caption{Research Model}
\label{tab:main_simplified}
\vspace{3pt}
\resizebox{0.8\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\ 
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\ 
 & \textbf{F1} & \textbf{F1} & \textbf{F1} &  & \\
\hline
\textsc{Qwen2.5 0.5B}  & 10.03 & 11.14 & 11.64 & 3.50 & 9.08\\
\textsc{Qwen2.5 3B}    & 39.76 & 37.16 & 33.04 & 23.96 & 33.48\\
\textsc{Qwen2.5 7B}    & 51.95 & 47.95 & 48.55 & 26.93 & 43.85\\
\textsc{Qwen2.5 14B}   & 64.07 & 55.99 & 57.87 & 34.77 & 53.18\\
\textsc{Qwen2.5 32B}   & 61.93 & 59.19 & 61.53 & 35.33 & 54.50\\
\textsc{GPT-4o-mini}   & 62.06 & 62.97 & 61.54 & 35.24 & 55.45 \\
\hline
\end{tabular}%
}
\end{table*}





\begin{table*}[htbp]
\centering
\caption{Efficiency on HotpotQA}
\label{tab:efficiency}
\vspace{3pt}
\resizebox{0.8\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llccccc}
\hline
\textbf{Dataset} &
\textbf{Metric} &
\textbf{A-mem} &
\textbf{Mem0} &
\textbf{MemoryOS} &
\textbf{LightMem} &
\textbf{GAM} \\
\hline
\multirow{3}{*}{\textbf{HotpotQA 56k}} 
  & \textsc{Memorize}            & 209.74 & 37.42  & 80.36 & 4.93 & 56.89 \\
  & \textsc{Search \& Answer}    & 0.52   & 0.15   & 0.44  & 0.20 & 12.43 \\
  & \textsc{All}                 & 210.26 & 37.57  & 80.80 & 5.13 & 69.32 \\
\hline
\multirow{3}{*}{\textbf{HotpotQA 224k}} 
  & \textsc{Memorize}            & 904.99  & 165.30  & 325.70 & 16.61    & 252.72 \\
  & \textsc{Search \& Answer}    & 0.48  & 0.17  & 3.42   & 0.25     & 16.65  \\
  & \textsc{All}                 & 905.46  & 165.47  & 329.12 & 16.86    & 269.37 \\
\hline
\multirow{3}{*}{\textbf{HotpotQA 448k}} 
  & \textsc{Memorize}            & 1796.82  & 274.87  & 702.72 & 40.56  & 557.16 \\
  & \textsc{Retrieve \& Answer}    & 0.47  & 0.18  & 0.46 & 0.21   & 18.49  \\
  & \textsc{All}                 & 1797.29 & 275.05 & 703.18  & 40.78  & 575.65 \\
\hline


\end{tabular}%
}
\end{table*}

% \cline{2-6}
% & \textbf{56K} & \textbf{224K} & \textbf{448K} & \multirow{2}{*}{\textbf{F1}} & \multirow{2}{*}{\textbf{F1}} \\ 
%  & \textbf{F1} & \textbf{F1} & \textbf{F1} &  & \\
% \hline

% \textsc{Qwen2.5 3B}    & 39.76 & 37.16 & 33.04 & 23.96 & 33.48\\
% \textsc{Qwen2.5 7B}    & 51.95 & 47.95 & 48.55 & 26.93 & 43.85\\
% \textsc{Qwen2.5 14B}   & 64.07 & 55.99 & 57.87 & 34.77 & 53.18\\
% \textsc{Qwen2.5 32B}   & 61.93 & 59.19 & 61.53 & 35.33 & 54.50\\
% \textsc{GPT-4o-mini}   & 62.06 & 62.97 & 61.54 & 35.24 & 55.45 \\




\begin{table*}[htbp]
\centering
\caption{Tools and Components Analysis}
\label{tab:tools_components}
\vspace{3pt}
\resizebox{0.6\textwidth}{!}{%
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{l|ccc|c|c}
\hline
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{3}{c|}{\textbf{HotpotQA}} &
\textbf{NarrativeQA} &
\textbf{Avg} \\ 
\cline{2-6}
& \textbf{56K} & \textbf{224K} & \textbf{448K} & \textbf{F1} & \textbf{F1} \\
\hline




\textsc{GAM}       & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\
\hline
\rowcolor{gray!20}
\multicolumn{6}{l}{\textbf{Tools Set}} \\
% \textsc{GAM}       & 64.07 & 55.99 & 57.87 & 34.77 & 53.18 \\

\quad \textsc{Only Page-id}          & 28.07 & 16.32 & 13.82 & 31.74 & 22.49 \\
\quad \textsc{Only Embedding}        & 38.57 & 31.38 & 27.09 & 32.08 & 32.28 \\
\quad \textsc{Only BM25}             & 59.79 & 53.58 & 49.91 & 31.78 & 48.77 \\
\quad \textsc{Embedding+Page-id}     & 42.41 & 30.35 & 29.54 & 33.84 & 34.04 \\
\quad \textsc{Embedding+BM25}        & 63.19 & 55.91 & 55.94 & 33.21 & 52.06 \\
\quad \textsc{BM25+Page-id}          & 63.52 & 55.29 & 55.93 & 33.50 & 52.06 \\

\hline

\rowcolor{gray!20}
\multicolumn{6}{l}{\textbf{Components}} \\


\quad \textsc{w/o Memory Planning}    & 57.40 & 49.72 & 53.98 & 31.97 & 48.27 \\
\quad \textsc{w/o Research Agent}     & 42.67 & 19.75 & 17.38 & 30.18 & 27.50 \\

\hline
\end{tabular}%
}
\end{table*}



==> table/scaling_test.tex <==
\begin{table*}[tb!]
\centering
\caption{Scaling results}
\label{tab:scaling}
\vspace{3pt}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|cccccccc|c}
\hline
\multicolumn{1}{c|}{\textbf{Model}} &
\multicolumn{8}{c|}{\textbf{LoCoMo}} &
LongMemEval \\ \cline{2-10}
& \multicolumn{2}{c}{\textbf{Single Hop}} & \multicolumn{2}{c}{\textbf{Multi Hop}} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c|}{\textbf{Open Domain}} & \\
& \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} & \textbf{F1} & \textbf{BLEU-1} &
\textbf{Acc.}  \\ 
\hline

\textbf{GPT-4o-mini} & 56.49 & 51.00 & 42.96 & 35.59 & 58.49 & 52.44 & 24.59 & 19.77 & 66.40 \\
\textbf{Qwen2.5 14b} & 57.09 & 51.62 & 42.55 & 34.98 & 40.96 & 35.09 & 24.27 & 19.23 & 61.80 \\
\textbf{Qwen2.5 7b}  & 57.80 & 52.70 & 36.65 & 28.82 & 35.43 & 29.75 & 22.44 & 17.75 & 48.40 \\ 
\textbf{Qwen2.5 3b}  & 45.26 & 40.52 & 29.30 & 22.69 & 32.90 & 27.63 & 14.90 & 11.12 & 41.60  \\ 
\hline

\end{tabular}%
}
\end{table*}

